Parallel and Asynchronous Smart Contract Execution

Today's blockchains suffer from low throughput and high latency, which impedes their widespread adoption of more complex applications like smart contracts. In this paper, we propose a novel paradigm for smart contract execution. It distinguishes between consensus nodes and execution nodes: different groups of execution nodes can execute transactions in parallel; meanwhile, consensus nodes can asynchronously order transactions and process execution results. Moreover, it requires no coordination among execution nodes and can effectively prevent livelocks. We show two ways of applying this paradigm to blockchains. First, we show how we can make Ethereum support parallel and asynchronous contract execution \emph{without hard-forks}. Then, we propose a new public, permissionless blockchain. Our benchmark shows that, with a fast consensus layer, it can provide a high throughput even for complex transactions like Cryptokitties gene mixing. It can also protect simple transactions from being starved by complex transactions.

==> sections/BFT.tex <==
%\section{BFT for $\name$ \dawn{we change the heading here.}}
\section{\BFT}
\label{sec:BFT}

%\dawn{I think we should give the BFT protocol a different name}
In this section, we propose a novel BFT protocol called $\BFT$ 
for the $\cons$ nodes in $\name$.  
It is of independent interest and can be used in any BFT-based applications.

\subsection{Overview}
\label{sec:BFT_overview}

%\dawn{this section is very confusing, since it's using different terminology now}
%Before describing $\BFT$, 
Before describing $\BFT$, we ask the question: 
{\em in PBFT~\cite{PBFT}, if all servers receive $3f+1$ matching $\prepareM$ messages in the prepare phase, do they still need a commit phase?}
The answer can be found in Zyzzyva~\cite{Zyzzyva} (and Zelma~\cite{abraham2018}): 
$3f+1$ matching replies suffice to convince the client 
%to complete its request.
that the position of its request in the history of correct servers is stable even 
when view-change happens.  
Therefore, we claim that $3f+1$ matching $\prepareM$ messages suffice to convince a server to execute the request as well. 
Based on this observation, we are able to build an optimistic protocol for free\footnote{Typically, optimistic protocols require clients participation, state rollback~\cite{Zyzzyva}, failure detection~\cite{FastBFT} or fallback protocol~\cite{Kapitza2012}. However, our protocol does not require any of them.}: 
if a server receives $3f+1$ matching $\prepareM$ messages in PBFT, it executes the request directly and replies to the client; otherwise (receiving between $2f+1$ and $3f$ $\prepareM$ messages), it moves to the commit phase waiting for $2f+1$ $\commitM$ messages to execute the request. 
%We call it $\BFT$ since it can be seen as a combination between Zyzzyva and PBFT.
Furthermore, we also adopt the signature aggregation technique in~\cite{Byzcoin} so that each non-primary server only needs to send and receive a single message for each step.
The communication pattern of $\BFT$ is shown in Fig.~\ref{fig:BFT}.
Its two-phase track is exactly the same as ByzCoin and ByzCoinX (\fig~\ref{fig:ByzCoin} in Appendix), but its fast track has one phase less.

%The intuition is to have the clients send their transactions to the primary $\Ser_p$, who forwards the ordered transactions to other $\Ser_i$s. 
%Each $\Ser_i$ replies a signature to $\Ser_p$ to signal that it agrees with the order. 
%We use multisignatures so that $\Ser_p$ can aggregate the signatures. %\asokan{If you want to use multisignatures (or even otherwise) you should say something about key management, especially since you want to claim that the scheme works for permission-less blockchains too.  Eg. how does the client learn the signature verification key? How does it get updated when Oi s join or leave }
%After gathering $3f+1$ valid signatures, $\Ser_p$ is able to convince all servers to execute the transactions. 
%To this end, $\Ser_p$ sends the aggregated signature to all servers. 
%After seeing the aggregated signature, all servers execute the transactions and reply to the clients.
%This will be the common-case scenario.


%If $\Ser_p$ receives between $2f+1$ and $3f$ valid signatures, it constructs a ``{\em commit certificate}'' by aggregating the signatures it has received, and forwards it to $\Ser_i$s.
%Once at least $2f+1$ $\Ser_i$s acknowledge receiving the commit certificate by replying with signatures,
%$\Ser_p$ aggregates these signatures and sends it again to all servers, who will execute the transactions and reply to the clients.
%Since this case requires a two-phase agreement, we call it the {\em two-phase track}, the communication pattern of which is shown in Fig.~\ref{fig:SaberBFTtwophase}.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[Fast track.]
    {
\begin{tikzpicture}
  [scale=.6,auto=center]
   \node at (1.1, 5.5) {\scriptsize \sf request};
   \node at (3, 5.5) {\scriptsize \sf pre-prepare};
   \node at (5.5, 5.5) {\scriptsize \sf prepare};
     \node at (8, 5.5) {\scriptsize \sf reply};

   \draw [thick, dotted] (1.9, 0.5) -- (1.9, 6);
    \draw [thick, dotted] (4.1, 0.5) -- (4.1, 6);
     \draw [thick, dotted] (7, 0.5) -- (7, 6);

   \node at (0,5) {$\Cli$};
   \draw [thick] (0.5,5) -- (9,5);
   \draw [->,shorten >=2pt,>=stealth] (0.6, 5) -- (1.9, 4);

    \node at (0,4) {$S_1$};
     \draw [thick] (0.5,4) -- (9,4);
     \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 3);
     \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.8, 2);
     \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.85, 1);
     
    \draw [->,shorten >=2pt,>=stealth] (5.6, 4) -- (6.9, 3);
    \draw [->,shorten >=2pt,>=stealth] (5.6, 4) -- (6.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (5.6, 4) -- (6.85, 1);
    
     \draw [->,shorten >=2pt,>=stealth] (7.1, 4) -- (8.7, 5);

   \node at (0,3) {$\Ser_2$};
   \draw [thick] (0.5,3) -- (9,3);
     \draw [->,shorten >=2pt,>=stealth] (4.1, 3) -- (5.3, 4);

      \draw [->,shorten >=2pt,>=stealth] (7.2, 3) -- (8.8, 5);

    \node at (0,2) {$\Ser_3$};
  \draw [thick] (0.5,2) -- (9,2);
     \draw [->,shorten >=2pt,>=stealth] (4.1, 2) -- (5.5, 4);

     \draw [->,shorten >=2pt,>=stealth] (7.3, 2) -- (8.9, 5);

    \node at (0,1) {$\Ser_4$};
    \draw [thick] (0.5,1) -- (9,1);
    \draw [->,shorten >=2pt,>=stealth] (4.2, 1) -- (5.6, 4);

%\draw [decorate,decoration={brace,amplitude=5pt}]
(2,6) -- (8,6) node %[black,midway,yshift=8]
%{\scriptsize {\bf Agreement}};

\end{tikzpicture}
        \label{fig:saberBFTfast}
    %    \vspace{-0.8 em}
    }\end{subfigure}
    
    \hspace{0.5in}

    \begin{subfigure}[Two-phase track.]
    {
\begin{tikzpicture}
  [scale=.6,auto=center]
   \node at (1.1, 5.5) {\scriptsize \sf request};
   \node at (3, 5.5) {\scriptsize \sf pre-prepare};
   \node at (5.5, 5.5) {\scriptsize \sf prepare};
    \node at (8.5, 5.54) {\scriptsize \sf commit};
     \node at (10.7, 5.5) {\scriptsize \sf reply};

   \draw [thick, dotted] (1.9, 0.5) -- (1.9, 6);
    \draw [thick, dotted] (4.1, 0.5) -- (4.1, 6);
     \draw [thick, dotted] (7, 0.5) -- (7, 6);
      \draw [thick, dotted] (10, 0.5) -- (10, 6);

   \node at (0,5) {$\Cli$};
   \draw [thick] (0.5,5) -- (11.5,5);
   \draw [->,shorten >=2pt,>=stealth] (0.6, 5) -- (1.9, 4);

    \node at (0,4) {$\Ser_1$};
     \draw [thick] (0.5,4) -- (11.5,4);
     \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 3);
     \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.8, 2);
     \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.85, 1);
     
    \draw [->,shorten >=2pt,>=stealth] (5.6, 4) -- (6.9, 3);
    \draw [->,shorten >=2pt,>=stealth] (5.6, 4) -- (6.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (5.6, 4) -- (6.85, 1);
     

     \draw [->,shorten >=2pt,>=stealth] (8.6, 4) -- (9.9, 3);
     \draw [->,shorten >=2pt,>=stealth] (8.6, 4) -- (9.6, 2);
     \draw [->,shorten >=2pt,>=stealth] (8.6, 4) -- (9.4, 1);

     \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.2, 5);

   \node at (0,3) {$\Ser_2$};
   \draw [thick] (0.5,3) -- (11.5,3);
     \draw [->,shorten >=2pt,>=stealth] (4.1, 3) -- (5.3, 4);

     \draw [->,shorten >=2pt,>=stealth] (7.3, 3) -- (8.5, 4);

      \draw [->,shorten >=2pt,>=stealth] (10.4, 3) -- (11.3, 5);

    \node at (0,2) {$\Ser_3$};
  \draw [thick] (0.5,2) -- (11.5,2);
     \draw [->,shorten >=2pt,>=stealth] (4.1, 2) -- (5.5, 4);

     \draw [->,shorten >=2pt,>=stealth] (7.2, 2) -- (8.6, 4);

     \draw [->,shorten >=2pt,>=stealth] (10.5, 2) -- (11.45, 5);

    \node at (0,1) {$\Ser_4$};
    \draw [thick] (0.5,1) -- (11.5,1);
    \node at (1.5, 1) {$\xmark$};

%\draw [decorate,decoration={brace,amplitude=5pt}]
(2,6) -- (8,6) node %[black,midway,yshift=8]
%{\scriptsize {\bf Agreement}};

\end{tikzpicture}
        \label{fig:SaberBFTtwophase}
    %    \vspace{-0.8 em}
    }\end{subfigure}
    \caption{Communication pattern in $\BFT$.}
    \label{fig:BFT}
\end{figure}

Next, we describe the normal-case and view-change operations as a reactive system (\fig~\ref{fig:saberBFT_normal_case} and \fig~\ref{fig:SaberBFT_view_change}). 
For the sake of brevity, we do not explicitly show the sequence number and signature verification.
We assume that each node verifies them for any message received as input.
%\dawn{we should consider putting Dagger in a separate paper; and just reference Dagger in this paper.}

\subsection{Normal-case operation}
\label{sec:normal-case}

%\noindent\textbf{Request.}
The normal-case operation of $\BFT$ is shown in \fig~\ref{fig:saberBFT_normal_case}.
A client requests the execution of a transaction $\trans$ by sending a signed request $M = \langle \request, \trans, \sigma_{\Cli} \rangle$ to $\Ser_p$. %where 
If it receives no reply after a timeout, it sends $M$ again to all $\Ser_i$s.
%\noindent\textbf{Preprepare.}
Upon receiving $M$, $\Ser_p$ assigns a sequence number $sn$ to $M$ by signing $\langle H(M), sn, v \rangle$ (line~\ref{2}) where $v$ is the current view number. 
The sequence number is monotonic increasing across different views.
Then, $\Ser_p$ multicasts $\langle \preprepare, M, sn, v, \sigma_{p} \rangle$ to all $\Ser_i$s (line~\ref{3}).
%At this point, the request $M$ is {\em prepared}.
%\noindent\textbf{Prepare.}
Upon receiving the $\preprepareM$ message from $\Ser_p$, each $\Ser_i$ signs $\langle H(M), sn, v \rangle$ as well (line~\ref{6}), and replies to $\Ser_p$ with $\langle \prepare, H(M), sn, v, \sigma_{i} \rangle$ to signal that it agrees with the order (line~\ref{7}).

If $\Ser_p$ receives all $3f+1$ $\prepareM$ messages, 
it aggregates the received signatures into a single one $\widetilde{\sigma}_1$ (line~\ref{10}), and multicasts $\langle \prepared, H(M), sn, v, \widetilde{\sigma}_1 \rangle$ to all $\Ser_i$s (line~\ref{11}). 
The $\preparedM$ message is referred to as the {\em commit certificate}.
Upon receiving the $\preparedM$ message from $\Ser_p$, 
each $\Ser_i$ executes $\trans$ (line~\ref{20}) and signs the result $res$ (line~\ref{21}).
Then each $\Ser_i$ replies to $\Cli$ with $\langle \reply, H(M), sn, \sigma''_{i}, v \rangle$ (line~\ref{22}).

If $\Ser_p$ receives between $2f+1$ and $3f$ $\prepareM$ messages (line~\ref{14}), it also aggregates the received signatures into a single one $\widetilde{\sigma}_2$ (line~\ref{15}) and multicasts $\langle \commitrequest, H(M), sn, v,  \widetilde{\sigma}_2 \rangle$ to all $\Ser_i$s (line~\ref{34}).
Upon receiving the $\commitrequestM$ message from $\Ser_p$, each $\Ser_i$
does the same thing as they did for $\preprepareM$ and replies to $\Ser_p$ with $\langle \commit, H(M), sn, v, \sigma'_{i} \rangle$ (line~\ref{17}-\ref{18}).
Upon receiving at lest $2f+1$ $\commitM$ messages, $\Ser_p$ does the same thing as they did for $\prepareM$ and multicasts $\langle \committed, H(M), sn, v, \widetilde{\sigma}_2, \widetilde{\sigma}'_2 \rangle$ to all $\Ser_i$s (line~\ref{23}-\ref{24}). 
Upon receiving the $\committedM$ message from $\Ser_p$, each $\Ser_i$ executes $\trans$ and replies to the client (line~\ref{27}-\ref{29}).

In either track, the client waits for $f+1$ consistent replies to accept the result.

\begin{figure}[htbp]
\small
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]

%--------------------------------
\State \textbf{upon} reception of $M = \langle \request, \trans, \sigma_{\Cli} \rangle$ at $\Ser_p$ \textbf{do}
\State\label{2} \phantom{----} $\sigma_{p}$ $\leftarrow$ \sign($\langle H(M), sn, v \rangle$)
\State\label{3} \phantom{----} multicast $\langle \preprepare, M, sn, v, \sigma_{p} \rangle$ to all $\Ser_i$s
\\

%--------------------------------
\State \textbf{upon} reception of $\langle \preprepare, M, sn, v, \sigma_{p} \rangle$ at $\Ser_i$ \textbf{do}
%\State\label{13} \phantom{----} \textbf{if} $c$ is sequential
\State\label{6} \phantom{----} $\sigma_{i}$ $\leftarrow$ \sign($\langle H(M), sn, v \rangle$)
\State\label{7} \phantom{----} send $\langle \prepare, H(M), sn, v, \sigma_{i} \rangle$ to $\Ser_p$
\\

%--------------------------------
\State \textbf{upon} reception of $(3f+1)$ $\langle \prepare, H(M), sn, v, \sigma_{i} \rangle$s at $\Ser_p$ \textbf{do}
%\State\label{15} \phantom{----} $\widetilde{\sigma}_1$ \leftarrow$ \aggregate($\sigma_{o_1}, ..., \sigma_{o_n}$) 
\State\label{10} \phantom{----} $\widetilde{\sigma}_1 \leftarrow$ \aggregate($\{\sigma_{i}\}_n$) 
\State\label{11} \phantom{----} multicast $\langle \prepared, H(M), sn, v, \widetilde{\sigma}_1 \rangle$ to all $\Ser_i$s

\\


%--------------------------------
\State\label{13} \textbf{upon} reception of $\langle \prepared, H(M), sn, v, \widetilde{\sigma}_1 \rangle$ at $\Ser_i$ \textbf{do}
%\State\label{13} \phantom{----} \textbf{if} $c$ is sequential
\State\label{20}\phantom{-----} $res$ $\leftarrow$ Execute $\trans$
\State\label{21} \phantom{----} $\sigma''_{i}$ $\leftarrow$ \sign($\langle H(res), sn, v$)
\State\label{22} \phantom{----} send $\langle \reply, res, sn, v, \sigma''_{i} \rangle$ to $\Cli$
\\

%--------------------------------
\State \textbf{upon} timeout at $\Ser_p$ \textbf{do}
\State\label{14} \phantom{----} \textbf{if} received at least $(2f+1)$ $\langle \prepare, H(M), sn, v, \sigma_{i} \rangle$s
%\State\label{13} \phantom{----}\phantom{----} $\widetilde{\sigma}_2$ \leftarrow$ \aggregate($\sigma_{o_1}, ... \sigma_{o_{2f+1}}$)
\State\label{15} \phantom{----}\phantom{---} $\widetilde{\sigma}_2 \leftarrow$ \aggregate($\{\sigma_{i}\}_{2f+1}$) 

\State\label{34} \phantom{----}\phantom{---} multicast $\langle \commitrequest, H(M), sn, v, \widetilde{\sigma}_2 \rangle$ to $\Ser_i$s
\State\label{35} \phantom{----} \textbf{else}
\State\label{36} \phantom{----}\phantom{---} multicast $\langle \preprepare, M, sn, v, \sigma_{p} \rangle$ to $\Ser_i$s
\\

%--------------------------------
\State \textbf{upon} reception of $\langle \commitrequest, H(M), sn, v, \widetilde{\sigma}_2 \rangle$ at $\Ser_i$ \textbf{do}
%\State\label{13} \phantom{----} \textbf{if} $c$ is sequential
\State\label{17} \phantom{----} $\sigma'_{i}$ $\leftarrow$ \sign($\langle H(M), sn, v, \commit \rangle$)
\State\label{18} \phantom{----} send $\langle \commit, H(M), sn, v, \sigma'_{i} \rangle$ to $\Ser_p$
\\

%--------------------------------
\State \textbf{upon} reception of $(2f+1)$ $\langle \commit, H(M), sn, v, \sigma'_{i} \rangle$s at $\Ser_p$ \textbf{do}

\State\label{23} \phantom{----} $\widetilde{\sigma}'_2 \leftarrow$ \aggregate($\{\sigma'_{i}\}_{2f+1}$) 
%\State\label{27} \phantom{----}\phantom{----} multicast $\langle \ord, M, c, \widetilde{\sigma}_2, \widetilde{\sigma}'_2 \rangle$ to all $\exec_i$s
\State\label{24} \phantom{----} multicast $\langle \committed, M, sn, v, \widetilde{\sigma}_2, \widetilde{\sigma}'_2 \rangle$ to $\Ser_i$s
\\

%--------------------------------
\State\label{26} \textbf{upon} reception of $\langle \committed, M, sn, v, \widetilde{\sigma}_2, \widetilde{\sigma}'_2 \rangle$ at $\Ser_i$ \textbf{do}
%\State\label{13} \phantom{----} \textbf{if} $c$ is sequential
\State\label{27}\phantom{-----} $res$ $\leftarrow$ Execute $\trans$
\State\label{28} \phantom{----} $\sigma''_{i}$ $\leftarrow$ \sign($\langle H(res), sn, v$)
\State\label{29} \phantom{----} send $\langle \reply, res, sn, v, \sigma''_{i} \rangle$ to $\Cli$

\end{algorithmic}
\end{mdframed}
\caption{Pseudocode: normal-case operations for $\BFT$.} %\asokan{show Sp and Si separately as two subfigures}
\label{fig:saberBFT_normal_case}
\end{figure}


\subsection{View-change}
\label{sec:view-change}

Recall that the client sets a timer after sending the request to $\Ser_p$. 
It will send the request to all $\Ser_i$s if no reply was received after the timeout.
After receiving the request from the client, each $\Ser_i$ will also set a timer. 
If $\Ser_i$ receives no message from $\Ser_p$ before the timeout,
it will initialize a view-change by broadcasting a $\langle \reqviewchange, v \rangle$ message. 
In addition, $\Ser_i$ can also suspect that $\Ser_p$ is faulty by verifying the messages it received and initialize a view-change. 

%The view-change operation must elect a new primary $\Ser_{p'}$ and guarantee that it will not introduce any changes in the history.
The view-change operation of $\BFT$ is shown in \fig~\ref{fig:SaberBFT_view_change}.
Upon receiving at least $f+1$ $\reqviewchangeM$ messages, $\Ser_i$ constructs a message log and multicasts it to others inside a $\viewchangeM$ message (line~\ref{2.2}-\ref{2.3}). 
After receiving at least $2f+1$ $\viewchangeM$ messages, the new primary $\Ser_{p'}$ construct a global message log $\widetilde{L}$ based on the received message logs (line~\ref{2.8}-\ref{2.16}).
%Note that the attack to Zyzzyva pointed out by Abraham et al.~\cite{abraham2017} applies to $\BFT$ as well.  
Here, we follow the strategy provided by~\cite{abraham2017}: if there are conflicts between the fast track decision and the two-phase track decision (line~\ref{2.12}), $\Ser_i$ follows the one with higher view number (line~\ref{2.13}).
Upon receiving the $\newviewM$ message, each $\Ser_i$ verifies $\widetilde{L}$ by constructing it again (line~\ref{2.21}). 
Then, each $\Ser_i$ updates its state by executing the transactions in $\widetilde{L}$ it has not executed before (line~\ref{2.22}). 
In the end, all servers switch to the next view. 
%\dawn{can we use Solida or similar approach in dfinity to just rotate the leader periodically, leveraging an underlying PoW chain?}

\begin{figure}[htbp]
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]
\small

\State \textbf{upon} reception of at least $f+1$ $\langle \reqviewchange, v \rangle$s at $\Ser_i$ \textbf{do}
\State\label{2.2} \phantom{---}
construct a message log $L$ that includes all $\preprepare$, $\commitrequest$ and $\committed$ messages it has received since the latest stable checkpoint\footnote{\scriptsize{Similarly to other BFT protocols, $\BFT$ generates checkpoints periodically to limit the number of messages in the log.}}
\State\label{2.3} \phantom{---}
$\sigma_{i}$ $\leftarrow$ \sign($\langle H(L)\rangle$)
\State\label{2.4} \phantom{---}
multicast $\langle \viewchange, v+1, L, \sigma_{i}\rangle$ to others
\\

%--------------------
\State \textbf{upon} reception of at least $2f+1$  $\langle \viewchange, v+1, L, \sigma_{i}\rangle$s at $\Ser_{p'}$ \textbf{do}
\State\label{2.7}\phantom{----}set $\widetilde{L}$ as an empty log \Comment{construct a global message log $\widetilde{L}$} %based on $\{L\}$}
\State\label{2.8}\phantom{----}\textbf{for} each $sn$ \Comment{from the smallest $sn$ since the checkpoint}
\State\label{2.9}\phantom{----}\phantom{----} \textbf{if} there is a $\prepared$ %or\footnote{We will show that $\prepared$ and $\committed$ will not both appear for the same $sn$.} $\committed$ 
message for a $\preprepare$ message with $sn$
\State\label{2.10} \phantom{----}\phantom{----}\phantom{----} 
put that $\preprepare$ message into $\widetilde{L}$ and mark it as ``to be executed''
\State\label{2.11}\phantom{----}\phantom{----} \textbf{else if} there are $f+1$ matching $\preprepare$ messages with $sn$ AND
there is a $\commitrequest$ message for a different $\preprepare$ with $sn$ 
\State\label{2.12} \phantom{----}\phantom{----}\phantom{----}put the $\preprepare$ message {\bf with higher view number} into $\widetilde{L}$ and mark it as ``to be committed''
\State\label{2.13}\phantom{----}\phantom{----}\textbf{else if} there are $f+1$ matching $\preprepare$ messages with $sn$ 
\State\label{2.14} \phantom{----}\phantom{----}\phantom{----}put that $\preprepare$ message into $\widetilde{L}$ and mark it as ``to be committed''
\State\label{2.15}\phantom{----}\phantom{----}\textbf{else if}
there is a $\commitrequest$ message for a  $\preprepare$ with $sn$ 
\State\label{2.16} \phantom{----}\phantom{----}\phantom{----}put that $\preprepare$ message into $\widetilde{L}$ and mark it as ``to be committed''

\State\label{2.17}\phantom{---}
$\sigma_{p'}$ $\leftarrow$ \sign($\langle H(\widetilde{L})\rangle$)

\State\label{2.18}\phantom{----}multicast $\langle \newview, v+1, \widetilde{L}, \sigma_{p'} \rangle$ to all $\Ser_i$s
\\

%--------------------
\State \textbf{upon} reception of $\langle \newview, v+1, \widetilde{L}, \sigma_{p'} \rangle$ at $\Ser_{i}$ \textbf{do}
\State\label{2.21}\phantom{----}verify $\widetilde{L}$ in the same way as it was constructed
\State\label{2.22}\phantom{----}execute the transactions in $\widetilde{L}$ that are marked as ``to be executed''
\State\label{2.23}\phantom{----}switch to the next view to commit and execute the transactions in $\widetilde{L}$ that are marked as ``to be committed''

\end{algorithmic}
\end{mdframed}
\caption{Pseudocode: view-change operation for $\BFT$.}
\label{fig:SaberBFT_view_change}
\vspace{-0.18em}
\end{figure}

The safety and liveness arguments of $\BFT$ are discussed in Appendix~\ref{sec:argument}. 
We will include a formal proof in an extended version of this paper.

==> sections/BO.tex <==
\section{Byzantine Ordering}
\label{sec:bo}

Similar to state machine replication, a Byzantine ordering (BO) service is replicated across $n$ ordering nodes $\order_i$. 
Each node maintains an ordered list of transactions, 
receives new transactions from clients,
appends them to the list, 
and returns {\em sequence numbers} corresponding to the positions of these transactions in the list.
A client {\em completes} its request if it has received enough matching sequence numbers from different nodes.
A BO protocol should satisfy:
\begin{itemize}
\item {\em Safety}: all non-faulty nodes maintains transactions in the same order. 
\item {\em Liveness}: clients eventually complete their requests.
\end{itemize}

We provide an efficient BO instantiation. 
The intuition is to have the clients send their transactions to the primary $\order_p$, who forwards the ordered transactions to other $\order_i$s. 
Each $\order_i$ replies a signature to $\order_p$ to signal that it agrees with the order. 
We use multisignatures so that $\order_p$ can aggregate the signatures and send a single message to the client.
After gathering $3f+1$ valid signatures, $\order_p$ is able to convince the client that its requests has been successfully ordered.
The communication pattern for this {\em fast track} is shown in Fig.~\ref{fig:gracious_BO}.  
This will be the common-case scenario.
If $\order_p$ receives between $2f+1$ and $3f$ valid signatures, it constructs a ``{\em commit certificate}'' by aggregating the signatures it has received, and forwards it to $\order_i$s.
Once at least $2f+1$ $\order_i$s acknowledge receiving the commit certificate by replying with signatures,
$\order_p$ aggregates these signatures and forward the result to the client together with the commit certificate. 
Since this case requires a two-phase agreement, we call it the {\em two-phase track}, the communication pattern of which is shown in Fig.~\ref{fig:failure_BO}.\asokan{If you want to use multisignatures (or even otherwise) you should say something about key management, especially since you want to claim that the scheme works for permission-less blockchains too.  Eg. how does the client learn the signature verification key? How does it get updated when Oi s join or leave }
This protocol is similar to Zyzzyva~\cite{Zyzzyva}, but requires neither rollbacks nor clients' participation.
\asokan{but you rely on client timeouts to trigger view change. what else does Zyzzyva rely on the clients }
\ray{Does this protocol inherit Zyzzyva's safety problems? See reference above}

%Apparently, a BO service can be built on top of any BFT protocol.
%We choose Zyzzyva~\cite{Zyzzyva} since it is known to be the most efficient one.
%However, recall that Zyzzyva has two drawbacks: it requires node to rollback executions if inconsistency appears; and it requires clients' participation to the protocol.
%In BO, $\order_i$ does not need to execute the requests, so no rollback is required. 
%To get rid of clients' participation, we have $\order_i$ reply a signature to $\order_p$ instead of to the client.




\begin{figure}[htbp]
    \label{fig:BO}
    \centering
    \begin{subfigure}[Fast track.]
    {
\begin{tikzpicture}[scale=0.54]
    \node at (0.9, 5.5) {\scriptsize \sf request};
    \node at (3, 5.5) {\scriptsize \sf preprepare};
    \node at (5.1, 5.5) {\scriptsize \sf prepare};
    \node at (7, 5.55) {\scriptsize \sf order};


    \draw [thick, dotted] (1.85, 0.5) -- (1.85, 6);
    \draw [thick, dotted] (4.15, 0.5) -- (4.15, 6);
    \draw [thick, dotted] (6, 0.5) -- (6, 6);


   \node at (-0.5,5) {$C$};
   \draw [thick] (0,5) -- (8,5);
   \draw [->,shorten >=2pt,>=stealth] (0.1, 5) -- (1.9, 4);

    \node at (-0.5,4) {$\order_1$};
    \draw [thick] (0,4) -- (8,4);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 3);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 1);
     
    \draw [->,shorten >=2pt,>=stealth] (6.1, 4) -- (7.9, 5);


   \node at (-0.5,3) {$\order_2$};
   \draw [thick] (0,3) -- (8,3);

   \draw [->,shorten >=2pt,>=stealth] (4.2, 3) -- (5.5, 4);

    \node at (-0.5,2) {$\order_3$};
    \draw [thick] (0,2) -- (8,2);

    \draw [->,shorten >=2pt,>=stealth] (4.3, 2) -- (5.7, 4);

    \node at (-0.5,1) {$\order_4$};
    \draw [thick] (0,1) -- (8,1);
    \draw [->,shorten >=2pt,>=stealth] (4.4, 1) -- (5.9, 4);
    
\end{tikzpicture}
        \label{fig:gracious_BO}
    %    \vspace{-0.8 em}
    }\end{subfigure}
    
    \hspace{0.5in}

    \begin{subfigure}[Two-phase track.]
    {
\begin{tikzpicture}[scale=.54]
    \node at (0.9, 5.5) {\scriptsize \sf request};
    \node at (3, 5.5) {\scriptsize \sf preprepare};
    \node at (5.1, 5.5) {\scriptsize \sf prepare};
    \node at (8, 5.55) {\scriptsize \sf commit};
    \node at (11, 5.55) {\scriptsize \sf order};

    \draw [thick, dotted] (1.85, 0.5) -- (1.85, 6);
    \draw [thick, dotted] (4.15, 0.5) -- (4.15, 6);
    \draw [thick, dotted] (6, 0.5) -- (6, 6);
  %  \draw [thick, dotted] (8, -2.5) -- (8, 6);
    \draw [thick, dotted] (10, 0.5) -- (10, 6);

   \node at (-0.5,5) {$C$};
   \draw [thick] (0,5) -- (12,5);
   \draw [->,shorten >=2pt,>=stealth] (0.1, 5) -- (1.9, 4);

    \node at (-0.5,4) {$\order_1$};
    \draw [thick] (0,4) -- (12,4);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 3);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 1);

    \draw [->,shorten >=2pt,>=stealth] (6, 4) -- (7.9, 3);
    \draw [->,shorten >=2pt,>=stealth] (6, 4) -- (7.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (6, 4) -- (7.7, 1);
    
    \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.9, 5);

    
   \node at (-0.5,3) {$\order_2$};
   \draw [thick] (0,3) -- (12,3);

    \draw [->,shorten >=2pt,>=stealth] (4.2, 3) -- (5.7, 4);
    \draw [->,shorten >=2pt,>=stealth] (8.1, 3) -- (9.7, 4);

    \node at (-0.5,2) {$\order_3$};
    \draw [thick] (0,2) -- (12,2);

    \draw [->,shorten >=2pt,>=stealth] (4.3, 2) -- (5.9, 4);
    \draw [->,shorten >=2pt,>=stealth] (8.2, 2) -- (9.9, 4);

    \node at (-0.5,1) {$\order_4$};
    \draw [thick] (0,1) -- (12,1);
    \node at (1.5, 1) {$\xmark$};
    
\end{tikzpicture}
        \label{fig:failure_BO}
    %    \vspace{-0.8 em}
    }\end{subfigure}
    \caption{Communication pattern of BO within a view.}
\end{figure}


Next, we describe the fast track, two-phase track and view-change operations as a reactive system (\fig~\ref{fig:bo_fast_normal} and \fig~\ref{fig:BO_view_change}). 
For the sake of brevity, we do not explicitly show the sequence number and signature verification.
We assume that each node verifies them for any message received as input.

\begin{figure}[htbp]
\small
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]

%--------------------------------
\State \textbf{upon} reception of $M = \langle \request, trans, \sigma_{\Cli} \rangle$ at $\order_p$ \textbf{do}
\State\label{2} \phantom{----} $\sigma_{o_p}$ $\leftarrow$ \sign($\langle H(M), c \rangle$)
\State\label{3} \phantom{----} multicast $\langle \preprepare, M, c, \sigma_{o_p} \rangle$ to all $\order_i$s
\\

%--------------------------------
\State \textbf{upon} reception of $\langle \preprepare, M, c, \sigma_{o_p} \rangle$ at $\order_i$ \textbf{do}
%\State\label{13} \phantom{----} \textbf{if} $c$ is sequential
\State\label{6} \phantom{----} $\sigma_{o_i}$ $\leftarrow$ \sign($\langle H(M), c \rangle$)
\State\label{7} \phantom{----} send $\langle \prepare, H(M), c, \sigma_{o_i} \rangle$ to $\order_p$
\\

%--------------------------------
\State \textbf{upon} reception of $(3f+1)$ $\langle \prepare, H(M), c, \sigma_{o_i} \rangle$s at $\order_p$ \textbf{do}
%\State\label{15} \phantom{----} $\widetilde{\sigma}_1$ \leftarrow$ \aggregate($\sigma_{o_1}, ..., \sigma_{o_n}$) 
\State\label{10} \phantom{----} $\widetilde{\sigma}_1$ \leftarrow$ \aggregate($\{\sigma_{o_i}\}_n$) 
%\State\label{11} \phantom{----} multicast $\langle \ord, M, c, \widetilde{\sigma}_1 \rangle$ to all $\exec_i$s
\State\label{11} \phantom{----} send $\langle \ord, M, c, \widetilde{\sigma}_1 \rangle$ to $C$

\\

%--------------------------------
\State \textbf{upon} timeout at $\order_p$ \textbf{do}
\State\label{14} \phantom{----} \textbf{if} received at least $(2f+1)$ $\langle \prepare, H(M), c, \sigma_{o_i} \rangle$s
%\State\label{13} \phantom{----}\phantom{----} $\widetilde{\sigma}_2$ \leftarrow$ \aggregate($\sigma_{o_1}, ... \sigma_{o_{2f+1}}$)
\State\label{15} \phantom{----}\phantom{----} $\widetilde{\sigma}_2$ \leftarrow$ \aggregate($\{\sigma_{o_i}\}_{2f+1}$) 

\State\label{16} \phantom{----}\phantom{----} multicast $\langle \commit, H(M), c, \widetilde{\sigma}_2 \rangle$ to all $\order_i$s
\State\label{17} \phantom{----} \textbf{else}
\State\label{18} \phantom{----}\phantom{----} multicast $\langle \preprepare, M, c, \sigma_{p} \rangle$ to all $\order_i$s
\\

%--------------------------------
\State \textbf{upon} reception of $\langle \commit, H(M), c, \widetilde{\sigma}_2 \rangle$ at $\order_i$ \textbf{do}
%\State\label{13} \phantom{----} \textbf{if} $c$ is sequential
\State\label{21} \phantom{----} $\sigma'_{o_i}$ $\leftarrow$ \sign($\langle H(M), c, \commit \rangle$)
\State\label{22} \phantom{----} send $\langle \commit, H(M), c, \sigma'_{o_i} \rangle$ to $\order_p$
\\

%--------------------------------
\State \textbf{upon} reception of at least $(2f+1)$ $\langle \commit, H(M), c, \sigma'_{o_i} \rangle$s at $\order_p$ \textbf{do}

\State\label{25} \phantom{----}   \textbf{if} $\langle \ord, M, c, \widetilde{\sigma}_1 \rangle$  has not been sent
\State\label{26} \phantom{----}\phantom{----} $\widetilde{\sigma}'_2$ \leftarrow$ \aggregate($\{\sigma'_{o_i}\}_{2f+1}$) 
%\State\label{27} \phantom{----}\phantom{----} multicast $\langle \ord, M, c, \widetilde{\sigma}_2, \widetilde{\sigma}'_2 \rangle$ to all $\exec_i$s
\State\label{27} \phantom{----}\phantom{----} send $\langle \ord, M, c, \widetilde{\sigma}_2, \widetilde{\sigma}'_2 \rangle$ to $C$

\end{algorithmic}
\end{mdframed}
\caption{Pseudocode: fast-case and normal-case operations for BO\asokan{show Op and Oi separately as two subfigures}}
\label{fig:bo_fast_normal}
\end{figure}

\noindent\textbf{Request.}
A client requests the order of a transaction $trans$ by sending a signed request $M = \langle \request, trans, \sigma_{\Cli} \rangle$ to $\order_p$. %where 
If it receives no reply before a timeout, it sends $M$ again to all $\order_i$s.

\noindent\textbf{Preprepare.}
Upon receiving $M$, $\order_p$ assigns a sequence number $sn$ to $M$ by signing $\langle H(M), sn \rangle$ (line~\ref{2}).
Then, $\order_p$ multicasts $\langle \preprepare, M, sn, \sigma_{o_p} \rangle$ to all $\order_i$s (line~\ref{3}).
%At this point, the request $M$ is {\em prepared}.

\noindent\textbf{Prepare.}
Upon receiving the $\preprepare$ message from $\order_p$, each $\order_i$ signs $\langle H(M), sn \rangle$ as well (line~\ref{6}), and reply to $\order_p$ with $\langle \prepare, H(M), sn, \sigma_{o_i} \rangle$ to signal that it agrees with the order (line~\ref{7}).

\noindent\textbf{Commit.}
Suppose $\order_p$ receives between $2f+1$ and $3f$ $\prepare$ messages, 
it aggregates the received signatures into a single one (line~\ref{15}), 
and multicasts $\langle \commit, H(M), c, \widetilde{\sigma}_2 \rangle$ to all $\order_i$s (line~\ref{16}).
Upon receiving the $\commit$ message from $\order_p$, 
each $\order_i$ signs $\langle H(M), c, \commit \rangle$ (line~\ref{21})
and replies $\langle \commit, H(M), c, \sigma'_{o_i} \rangle$ to $\order_p$ (line~\ref{22}).


\noindent\textbf{Order.}
Upon receiving $3f+1$ $\prepare$ messages (line~\ref{10}) or at least $2f+1$ $\commit$ messages,
$\order_p$ aggregates all signatures into a single one,
and send $\langle \ord, M, sn, \widetilde{\sigma}_1 \rangle$ (line~\ref{11}) or $\langle \ord, M, sn, \widetilde{\sigma}_2, \widetilde{\sigma}'_2 \rangle$ (line~\ref{27}) to the client.

\noindent{\bf View-change}
Recall that the client sets a timer after sending a request to $\order_p$. 
It will send the request to all $\order_i$s if no reply was received before the timeout.
If a replica receives no $\prepare$ (or $\commit/\reply$) message before the timeout,
it will initialize a view-change (\fig~\ref{fig:BO_view_change}) by broadcasting a $\langle \reqviewchange, v \rangle$ message.
In addition, nodes can also suspect that $\order_p$ is faulty by verifying the messages they received and initialize a view-change.
Abraham et al. point out a safty violation in the view-change of Zyzzyva: 
a possible decision is transferred across views in two ways, corresponding to the two tracks, and combining them requires care~\cite{abraham2017}.
They also propose a fix by having a node accept a proposal in a new view as safe only if it is compatible with a potential decision from the highest view-number of any lower view~\cite{abraham2018}. 
We follow this strategy in our view-change operation.

\begin{figure}[htbp]
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]
\small

\State \textbf{upon} reception of at least $f+1$ $\langle \reqviewchange, v \rangle$s at $\order_i$ \textbf{do}
\State\label{2.13.2} \phantom{----} broadcast $\langle \viewchange, v+1, L, \sigma_{i}\rangle$, where $L$ is the message log  that includes all messages it has received/sent since the latest checkpoint
%\footnote{\scriptsize{Similar to other BFT protocols, \BFT generates checkpoints periodically to limit the number of messages in the log.}}.}
\\

%--------------------
\State \textbf{upon} reception of at least $2f+1$  $\langle \viewchange, v+1, L, \sigma_{i}\rangle$s at $\order_{p'}$ \textbf{do}
\State\label{2.6} \phantom{----} build a global message log $O$ based on message logs $\{L\}$
\State\label{2.10} \phantom{----} broadcast $\langle \newview, v+1, O, P, \sigma_{p'} \rangle$, where $P$ is the set containing valid $\viewchange$ messages for view $v+1$
\\

%--------------------
\State \textbf{upon} reception of $\langle \newview, v+1, O, P, \sigma_{p'} \rangle$ at $\order_{i}$ \textbf{do}
\State\label{2.13} \phantom{----} {\bf if} both $O$ and $P$ are valid
\State\label{2.13.3} \phantom{----}\phantom{----} update its sequence number to the latest

\end{algorithmic}
\end{mdframed}
\caption{Pseudocode: view-change operation for BO.}
\label{fig:BO_view_change}
\vspace{-0.18em}
\end{figure}



%\section{Separating agreement from execution: a new instantiation}
\section{Byzantine Fault Tolerance}
\label{sec:new_bft}

%We first consider the case where there is only a single shard,
%and leave the multi-shard case to the next section.
%Then, it matches exactly the architecture of ``separating agreement from execution''. 
%So, we can simply follow the approach in Yin et al.~\cite{Yin2003} by having $n=3f+1$ ordering nodes in the ordering committee run a standalone BFT protocol to order clients' requests, 
%and having $n'=2f'+1$ executing nodes in the shard execute the requests in the order determined by the ordering nodes (cf. Section~\ref{sec:bft}). 

The communication pattern is shown in \fig~\ref{}.
We rely on the BO service in Section~\ref{sec:bo} to build our BFT protocol.
So, the request, preprepare, prepare commit and order phase are exactly the same as they are in Figure~\ref{fig:bo_fast_normal}, 
except that in Line~\ref{11} and Line~\ref{27}, $\order_p$ sends the $\ord$ message to $\exec_i$s instead of $C$.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[Fast-case.]
    {
\begin{tikzpicture}[scale=0.54]
    \node at (0.9, 5.5) {\scriptsize \sf request};
    \node at (3, 5.5) {\scriptsize \sf preprepare};
    \node at (5.1, 5.5) {\scriptsize \sf prepare};
    \node at (7, 5.55) {\scriptsize \sf order};
    \node at (9, 5.55) {\scriptsize \sf execute};
    \node at (11, 5.5) {\scriptsize \sf reply};

    \draw [thick, dotted] (1.85, -2.5) -- (1.85, 6);
    \draw [thick, dotted] (4.15, -2.5) -- (4.15, 6);
    \draw [thick, dotted] (6, -2.5) -- (6, 6);
    \draw [thick, dotted] (8, -2.5) -- (8, 6);
    \draw [thick, dotted] (10, -2.5) -- (10, 6);

   \node at (-0.5,5) {$C$};
   \draw [thick] (0,5) -- (12,5);
   \draw [->,shorten >=2pt,>=stealth] (0.1, 5) -- (1.9, 4);

    \node at (-0.5,4) {$\order_1$};
    \draw [thick] (0,4) -- (12,4);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 3);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 1);
     
    \draw [->,shorten >=2pt,>=stealth] (6.1, 4) -- (7.9, 0);
    \draw [->,shorten >=2pt,>=stealth] (6.1, 4) -- (7.7, -1);
    \draw [->,shorten >=2pt,>=stealth] (6.1, 4) -- (7.6, -2);
    
    \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.8, 5);
    
    \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.8, 3);
    \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.8, 1);
    
   \node at (-0.5,3) {$\order_2$};
   \draw [thick] (0,3) -- (12,3);

   \draw [->,shorten >=2pt,>=stealth] (4.2, 3) -- (5.5, 4);

    \node at (-0.5,2) {$\order_3$};
    \draw [thick] (0,2) -- (12,2);

    \draw [->,shorten >=2pt,>=stealth] (4.3, 2) -- (5.7, 4);

    \node at (-0.5,1) {$\order_4$};
    \draw [thick] (0,1) -- (12,1);
    \draw [->,shorten >=2pt,>=stealth] (4.4, 1) -- (5.9, 4);
    
    \node at (-0.5, 0) {$\exec_1$};
    \draw [thick] (0,0) -- (12,0);
    \draw [->,shorten >=2pt,>=stealth] (8.1, 0) -- (9.7, 4);
    
    \node at (-0.5, -1) {$\exec_2$};
    \draw [thick] (0,-1) -- (12,-1);
    \draw [->,shorten >=2pt,>=stealth] (8.2, -1) -- (9.9, 4);
    
    \node at (-0.5, -2) {$\exec_3$};
    \draw [thick] (0,-2) -- (12,-2);
    \node at (1.5, -2) {$\xmark$};
    
\end{tikzpicture}
        \label{fig:gracious}
    %    \vspace{-0.8 em}
    }\end{subfigure}
    
    \hspace{0.5in}

    \begin{subfigure}[Normal-case.]
    {
\begin{tikzpicture}[scale=.54]
    \node at (0.9, 5.5) {\scriptsize \sf request};
    \node at (3, 5.5) {\scriptsize \sf preprepare};
    \node at (5.1, 5.5) {\scriptsize \sf prepare};
    \node at (8, 5.55) {\scriptsize \sf commit};
    \node at (11, 5.55) {\scriptsize \sf order};
    \node at (13, 5.55) {\scriptsize \sf execute};
    \node at (14.7, 5.5) {\scriptsize \sf reply};

    \draw [thick, dotted] (1.85, -2.5) -- (1.85, 6);
    \draw [thick, dotted] (4.15, -2.5) -- (4.15, 6);
    \draw [thick, dotted] (6, -2.5) -- (6, 6);
  %  \draw [thick, dotted] (8, -2.5) -- (8, 6);
    \draw [thick, dotted] (10, -2.5) -- (10, 6);
    \draw [thick, dotted] (12, -2.5) -- (12, 6);
    \draw [thick, dotted] (14, -2.5) -- (14, 6);

   \node at (-0.5,5) {$C$};
   \draw [thick] (0,5) -- (15.5,5);
   \draw [->,shorten >=2pt,>=stealth] (0.1, 5) -- (1.9, 4);

    \node at (-0.5,4) {$\order_1$};
    \draw [thick] (0,4) -- (15.5,4);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 3);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (2.1, 4) -- (3.9, 1);

    \draw [->,shorten >=2pt,>=stealth] (6, 4) -- (7.9, 3);
    \draw [->,shorten >=2pt,>=stealth] (6, 4) -- (7.8, 2);
    \draw [->,shorten >=2pt,>=stealth] (6, 4) -- (7.7, 1);
    
    \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.9, 0);
    \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.7, -1);
    \draw [->,shorten >=2pt,>=stealth] (10.1, 4) -- (11.6, -2);
    
    \draw [->,shorten >=2pt,>=stealth] (14.1, 4) -- (15.2, 5);
    \draw [->,shorten >=2pt,>=stealth] (14.1, 4) -- (15.2, 3);
    \draw [->,shorten >=2pt,>=stealth] (14.1, 4) -- (15.2, 2);
    \draw [->,shorten >=2pt,>=stealth] (14.1, 4) -- (15.2, 1);
    
   \node at (-0.5,3) {$\order_2$};
   \draw [thick] (0,3) -- (15.5,3);

    \draw [->,shorten >=2pt,>=stealth] (4.2, 3) -- (5.7, 4);
    \draw [->,shorten >=2pt,>=stealth] (8.1, 3) -- (9.7, 4);

    \node at (-0.5,2) {$\order_3$};
    \draw [thick] (0,2) -- (15.5,2);

    \draw [->,shorten >=2pt,>=stealth] (4.3, 2) -- (5.9, 4);
    \draw [->,shorten >=2pt,>=stealth] (8.2, 2) -- (9.9, 4);

    \node at (-0.5,1) {$\order_4$};
    \draw [thick] (0,1) -- (15.5,1);
    \node at (1.5, 1) {$\xmark$};
    
    \node at (-0.5, 0) {$\exec_1$};
    \draw [thick] (0,0) -- (15.5,0);
    \draw [->,shorten >=2pt,>=stealth] (12.1, 0) -- (13.7, 4);
    
    \node at (-0.5, -1) {$\exec_2$};
    \draw [thick] (0,-1) -- (15.5,-1);
    \draw [->,shorten >=2pt,>=stealth] (12.2, -1) -- (13.9, 4);
    
    \node at (-0.5, -2) {$\exec_3$};
    \draw [thick] (0,-2) -- (15.5,-2);
    \node at (1.5, -2) {$\xmark$};
    
\end{tikzpicture}
        \label{fig:failure}
    %    \vspace{-0.8 em}
    }\end{subfigure}
    
    
    \caption{Communication pattern for BFT within a view.}
\end{figure}

\begin{figure}[htbp]
\small
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]

%--------------------------------
\State \textbf{upon} reception of 
$\langle \ord, M, c, \widetilde{\sigma}_1 \rangle$ or 
$\langle \ord, M, c,$ 
$\widetilde{\sigma}_2,$ $\widetilde{\sigma}'_2 \rangle$ at $\exec_i$ \textbf{do}
%\State\label{13} \phantom{----} \textbf{if} $c$ is sequential
\State\label{30} \phantom{----} $\res$ $\leftarrow$ \execute($trans$)
\State\label{31} \phantom{----} $\sigma_{e_i}$ $\leftarrow$ \sign($\langle H(\res), c\rangle$)
\State\label{32} \phantom{----} send $\langle \reply, \res, c, \sigma_{e_i}\rangle$ to $\order_p$
\\

%--------------------------------
\State \textbf{upon} reception of at lest $(f'+1)$ $\langle \reply, \res, c, \sigma_{e_i}\rangle$s at $\order_p$ \textbf{do}
\State\label{35} \phantom{----} $\widetilde{\sigma}$ \leftarrow$ \aggregate($\{\sigma_{e_i}\}_{f'+1}$) 
\State\label{36} \phantom{----} multicast $\langle \reply, \res, c, \widetilde{\sigma} \rangle$ to all $\order_i$s and client

\end{algorithmic}
\end{mdframed}
\caption{Pseudocode: for BFT.}
\label{fig:view}
\end{figure}







\noindent\textbf{Execute.}
Upon receiving the $\ord$ message from $\order_p$, 
each $\exec_i$ executes $op$ (line~\ref{30}), sign the result (line~\ref{31}) and returns $\langle \reply, \res, c, \widetilde{\sigma} \rangle$ to $\order_p$ (line~\ref{32}).

\noindent\textbf{Reply.}
Upon receiving at least $2f'+1$ $\reply$ messages, 
$\order_p$ aggregates all signatures from $\exec_i$s (line~\ref{35}) and forwards the result to all $\order_i$s as well as the client (line~\ref{36}). 






%\subsection{Fast-case operation}

%\subsection{Normal-case operation}


%\subsection{Correctness arguments}

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discuss}

%\paragraph{Alternative separation}

\Paragraph{Other benefits of separation.} 
Separating execution from consensus has other benefits.
Since $\cons$ is generic (whereas execution is application specific), 
once execution has been separated from $\cons$,  application developers no longer need to worry about which consensus layer they are building on. 
Instead, they can develop an executable that can be run on any suitable consensus layer. 
%Our paradigm does not support this since it relies on $\order$s to do validity checking and lock handling.
Furthermore, institutions who have desires for private (consortium) blockchains can use an existing consensus layer as an ordering service, so that their nodes can execute the transactions without reaching any consensus.
For example, such institutions can join $\name$ as an ``execution group'' and have their users send transactions to the $\cons$ nodes, which will forward the ordered transactions to their ``execution nodes''.
The transactions can be encrypted so that they are only visible to their own nodes. %(not $\name$ nodes). 
In this case, institutions do not need to develop any consensus protocols for their private blockchains, and they only need to deploy $2f'+1$ nodes to tolerate $f'$ faults.

%Further more, correctness of execution does not necessarily depend on the consensus algorithm.
%For example, some executions can be done within trusted execution environments (TEEs) %~\cite{Ekiden}, 
%so that blockchain nodes only need to run consensus to agree on the transaction order instead of their execution results.
%\dawn{what's the point of this paragraph?}

%can use a generic blockchain for ordering but choose a different blockchain platform for execution. For example, they can use a private (e.g., enterprise-internal) blockchain if the smart contract they execute has confidential information. Or they can use a custom blockchain whose smart contract language allows specific computation (e.g., novel cryptographic operations) that are not supported by popular generic blockchains.


%\paragraph{Private (consortium) blockchain without consensus}\dawn{we should rename this differently}
%\dawn{it's not clear what benefit this brings. why would private blockchain want to use a public chain as a consensus layer?}
%Private (consortium) blockchains are maintained by a fixed set of nodes within one or several institutions, and the read/write permissions are restricted to a pre-defined set of users. 
%Customized consensus protocols are usually designed for such blockchains~\cite{hyperledger}. 
%We propose that institutions who have desires for private (consortium) blockchains can use an existing blockchain as an ordering service, so that their nodes can execute the transactions without reaching any consensus.
%\dawn{needs to bre rephrased. }
%\dawn{in this case, they don't have a private blockchain. }
%\paragraph{Penalty fee for locks}

\highlight{
\Paragraph{Gas model.} The gas model in traditional smart contracts is invalid for $\paradigm$ any more, since execution is no longer a bottleneck. 
The main bottleneck in $\paradigm$ is the lock handling and it leads to potential DoS attacks.
For example,
%reword
a malicious developer can create a smart contract in which he acquires all locks for all smart contracts, and sends a transaction for it once per round.  
This allows at most 1 execution group to make progress within that round since everybody has to wait. 
%-----------
We have to enforce more gas usage for such kind of smart contracts.
We leave designing a better gas model and incentive model for future work.
}

\Paragraph{Lock handling at compiler level.}
We rely on the smart contracts to handle locks, 
which require efforts from the contract developers. 
Developers are incentivized to reduce the gas consumption of their contracts.
However, it is clearly useful if we can provide assistants for lock handling at the compiler level, 
so that it is easier for the developers to develop their smart contracts.
We leave this as future work. %\pgao{This answers my questions on Page 6}

==> sections/full.tex <==
\section{Byzantine Sharding for Permissionless Blockchains}
\label{sec:full}

In a permissionless blockchain, nodes can join and leave at any time. Therefore, we need to be able to manage this dynamic membership.
Anyone can join the system by becoming a sybil-resistant identity.

In addition to the transaction blockchain, all nodes in the system maintain an {\em identity blockchain} to record the sybil-resistant identities, ordering nodes and executing nodes for all epochs.

To prevent an adaptive adversary from compromising more than a threshold number of
nodes in the ordering committee as well as in each shard, we need to swap them from the underlying sybil-resistant identities for each epoch.
This requires a random beacon to generate randomness that is unbiasable, unpredictable and third-party verifiable. 
We have the ordering committee run a randomness generation protocol  to simulate the random beacon.
We adopt the commit-and-reveal approach since it requires no configuration (cf. Section~\ref{sec:random}).

We assume that an initial ordering committee was chosen in the bootstrapping phase of the system, and it runs the randomness generation protocol to build all shards.
Then the ordering committee collaborates with those shards to process transactions.
After an epoch, the ordering committee runs the randomness generation protocol again to swap some ordering nodes and executing nodes.
Following OmniLedger~\cite{Omniledger}, we swap a subset of nodes to minimize the chances of a temporary loss of liveness.
After swapping, they move to the next epoch.



%\noindent{\bf Checkpointing.}




==> sections/overview.tex <==
\section{System Overview}

\subsection{System setting and assumptions}

Our system follows the setting of permissionless blockchains.
There are two main entities in the system: {\em clients} and {\em validators}. 
Clients are external entities who issue {\em transactions} to transfer funds or run smart contracts. 
Validators are the nodes in the network that process clients' transactions via a global consensus protocol. 
Notice that clients can play the role of validators and vice versa.  
In the rest of this paper, we use the terms validator and node interchangeably.
Each identity has a public/private key pair $(pk,sk)$ for a digital signature scheme, and we often identify an identity by its $pk$. 

Following previous work~\cite{BitcoinNG, Luu2016, Omniledger}, we assume that at most 25\% of the validators/nodes in the system can be Byzantine {\em at any point of time}.
We also assume that messages from honest nodes (in the absence of network partitions) can be delivered to honest destinations after a certain bound $\Delta$, which may be time-varying. 
As in PBFT~\cite{PBFT}, the bound $\Delta$  is used to ensure liveness but not safety.

\subsection{Design roadmap}

%We want to adopt the idea of Eris (cf. Section~\ref{sec:eris}) to build an efficient sharding protocol for permissionless blockchains. 
%However, Eris works in a permissioned setting and only tolerates crash faults. 


The Byzantine model leads to two challenges:
we cannot rely on a single sequencer to order requests since a Byzantine sequencer can equivocate;  
%assign the same counter value to different requests, or assign the same request with different counter values.
and we need to handle Byzantine faults within each committee, 
which thwarts the coordination-free property of Eris.

To overcome the first challenge, we introduce an {\em ordering committee} consists of $n$ nodes (called {\em ordering nodes $\order_i$}) 
\ray{There seem to be some missing symbols causing errors.}
to simulate the sequencer. 
Specifically, instead of sending requests to a single sequencer, 
clients send requests to the ordering committee
which runs a BFT protocol to 
impose a total order on transactions and assign a sequence number, consistent with the total order, to each transaction.
%ensure that  consistent sequence numbers are assigned to each request. 
Since BFT provides saftey and liveness, we no longer need a failure coordinator to handle sequencer failures and packet drops.

\ray{define $n'$?}
For the second challenge, we argue that it is enough to have all $n'$ nodes in each committee (called {\em executing nodes $\exec_i$}) directly execute the ordered requests without running a BFT protocol. This argument is based on the observation that our ordering committee plus a single committee exactly match the architecture of ``separating agreement from execution~\cite{Yin2003}'' (cf. Section~\ref{sec:bft}):
the ordering committee corresponds to the agreement cluster, 
and each committee corresponds to the execution cluster. 

In addition, we suggest that the ordering nodes do not need to run a full-fledged BFT protocol either, because they only order the requests instead of executing them.
To this end, we propose a new family of Byzantine protocols named as {\em Byzantine ordering} for the ordering committee, and provide an efficient instantiation for it.
Furthermore, we use the signature aggregation technique~\cite{CoSi} to make sure the message complexity is always linear.

The design roadmap leading to \name, our final blockchain protocol, is as follows:
\begin{enumerate}
\item We provide definition and an efficient instantiation for BO. (Section~\ref{sec:bo})
\item Based on our BO, we propose a novel BFT protocol following the architecture of ``separating agreement from execution''. (Section~\ref{sec:new_bft})
\item Based on our BFT, we propose a novel Byzantine protocol for permissioned blockchains. (Section~\ref{sec:sharding})
\item By adding dynamic membership management, we get our final protocol in permissionless blockchain setting. (Section~\ref{sec:full})
\end{enumerate}

\ray{I'm trying to understand the Byzantine ordering committee. Can you elaborate the intuition for why this is fast? It appears that you've introduced a timestamp server (implemented by a BFT committee) and a single bottleneck for all transactions. For crash fault systems (e.g. Eris), this can be implemented very quickly. But slowdowns by this committee are dramatically amplified. Will the system be limited by this committee?. In other sharding architectures, some allow parallel execution of transactions across independent objects. In Saber, are independent transactions are serialized by this committee?}

Notice that each of the protocols above is of independent interest. The system overview is shown in \fig~\ref{fig:overview}. We introduce notations as needed (summarized in Table~\ref{notationtable}).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{./pic/overview1} 
    \caption{System overview.}
    \label{fig:overview}
   % \emph{A note}
\end{figure}

\begin{table}[tb]
\small
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Notation} & \textbf{Description} \\ \hline

%\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Entities}} \\ \hline
%\multicolumn{2}{|l|} {\bf Entities} \\ \hline

%$\Cli$       & Client                      \\ \hline
$\order$      & ordering node                     \\ \hline
%USIG    &   Unique Sequential Identifier Generator  \\ \hline
%\multicolumn{2}{|l|} {\em \bf Objects} \\ \hline

%\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Objects}} \\ \hline
%$M$ & Request message \\ \hline
%$L$ &  Message Log \\ \hline
%$T$ &  Tree structure \\ \hline
%$\UI$	     &   Unique Identifier    \\ \hline
%$N$         &   Ephemeral nonce    \\  \hline

%\multicolumn{2}{|l|}{\em \bf Parameters} \\ \hline

%\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Parameters}} \\ \hline
$n$ & number of ordering nodes \\ \hline
$f$ &  number of faulty ordering nodes \\ \hline
$\exec$ & executing nodes  \\ \hline
$n'$ & number of executing nodes \\ \hline
$f'$ &  number of faulty executing nodes \\ \hline

$v$  & view number  \\ \hline
$sn$ & sequence number \\ \hline

%\multicolumn{2}{|l|}{\em \bf Cryptographic Notations} \\ \line

%\multicolumn{2}{|l|}{\cellcolor[HTML]{C0C0C0} {\em Cryptographic Notations}} \\ \hline
$H()$               &    cryptographic hash function \\ \hline
$h$               &     cryptographic hash             \\ \hline

$\sign() / \verify()$  & Signature generation / verification\\ \hline
$\sigma_$     & a Signature \\ \hline


\end{tabular}
\caption{Summary of notations}
\label{notationtable}
\vspace{-2 em}
\end{table}


==> sections/private.tex <==
\section{Private (Consortium) Blockchain as a Committee}

Private (consortium) blockchains are maintained by a fixed set of nodes within one or several institutions, and the read/write permissions are restricted to a pre-defined set of users. 
Customized consensus protocols are usually designed for such blockchains~\cite{hyperledger}. 
We propose that institutions who have desires for private (consortium) blockchains can use an existing blockchain as an ordering service, so that their nodes can execute the transactions without reaching any consensus.
For example, such institutions can join $\name$ as a ``committee'' and have their users send transactions to the ordering nodes, which will forward the ordered transactions to their ``execution nodes'' (\fig~\ref{fig:private}).
The transactions can be encrypted so that they are only visible to their own nodes. %(not $\name$ nodes).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{./pic/private} 
    \caption{Private/consortium blockchain as a committee.}
    \label{fig:private}
   % \emph{A note}
\end{figure}

==> sections/setting.tex <==




==> sections/sharding.tex <==
\section{Byzantine Sharding for Permissioned Blockchains}
\label{sec:sharding}

\subsection{Data model}

\subsubsection{Accounts and contracts}

Our system is an account-based system (as Ethereum). 
Each account is associated with an {\em account state}, which contains four fields:
\begin{enumerate}
\item account nonce:
\item balance:
\item contract code:
\item storage:
\end{enumerate}
There are two types of accounts: 
{\em normal account} controlled by private keys, 
and {\em contract account} controlled by their {\em contract code}.
By creating and signing a transaction, a normal account owner can simply transfer balance among normal accounts or 
invokes the code in contract accounts.

%A normal account has no code, and one can send messages from a normal account by creating and signing a {\em transaction}; 
%in a contract account, every time the contract account receives a message its code activates, allowing it to read and write to {\em internal storage} and send other messages or create contracts in turn.

Our sharding happens at accounts level.
Each account is identified by an {\em address}, 
based on which it is assigned to a single shard; 
each $e_i$ in that shard maintains a entire copy of its account state.
%each shard is responsible for multiple accounts, and each account state is maintained within a single shard.
%To support cross-shard transactions, each account has a {\em lock()} procedure that can be used to lock its balance or any other data objects in its storage.
\asokan{say how this is done. Using a deterministic function with a  uniform distribution?}

\subsubsection{Transactions, blocks and blockchains}
\label{sec:trans}

%Normal account owners (i.e., clients) use transactions to transfer balance or run smart contracts.
Transactions are sent from the normal account owners (i.e., clients) to the ordering committee, which then forwards the ordered transactions to the corresponding shards in the form of {\em blocks}.
%i.e., multiple transactions are grouped into a single block called {\em transaction block}.
We classify transactions into the following three categorizes:

\remove{
\begin{enumerate}
    \item {\em Single-shard transaction $\Trans_1$,} e.g., $A \rightarrow B$, which represents balance transfer between two normal accounts that are maintained in the same shard. 
    This kind of transactions can be committed in a single BFT round: the execution nodes simply check if $A$ has enough balance. If so, they commit the transaction, otherwise, they abort it.
    \item {\em Cross-shard independent transaction $\Trans_2$,} e.g., $A \rightarrow B$, where $A$ and $B$ are normal accounts maintained in different shards. In this case, the ordering nodes first make two single-shard transactions called {\em preliminary transactions} to check the balance of $A$ and try to lock both $A$ and $B$. Then, they make another single-shard transaction called {\em conclusory transaction} to either transfer the balance (if both transactions are committed), or release the lock (if one of them is aborted).
    \item {\em Transaction with cross-shard dependencies $\Trans_3$,} e.g., $A\rightarrow C\rightarrow B$, where $A$ and $B$ are normal accounts and $C$ is a contract account; $C\rightarrow B$ depends on the execution result of the contract code. This transaction is divided into two transactions $A\rightarrow C$ and $C\rightarrow B$ and process them separately.
\end{enumerate}
It is not difficult to see that all transactions can be divided into single-shard transactions.
}
%The ordering committee is responsible for gathering transactions, agreeing on their orders, and forwarding the ordered transactions to the corresponding shards.
%The ordered transactions are forwarded in the form of {\em blocks}, 

%Next, each $o_i$ combines the transaction block and the result block into a {\em final block}, and put it into its local {\em transaction blockchain}.
%Instead of replying to each individual client, results are put into the blockchain and 

In the end, the ordering nodes put both transactions and their execution result to the {\em transaction blockchain}.
\Jian{Should we put intermediate results in to the blockchain?}
Clients can fetch for the results from any $o_i$. 

\subsection{Sharding}


To support sharding, we have the ordering committee maintain a separate sequence number for each of the $m$ shards: $\langle sn_1, …, sn_m \rangle$.
%Given a request $M$, the ordering committee identifies its targeting shard $S_i$,  generates an $\ord$ message with the latest sequence number $sn_i$ for that shard, and send it to all $e_i$s.
%In blockchain setting, multiple requests are usually batched into a signal block and processed in a single BFT round.
%Recall that a cross-shard transaction can be divided into multiple single-shard transactions.
After gathering enough transactions, $\order_p$ builds $m$ blocks $\langle B_1, …, B_m\rangle$ following the pseudocode in \fig~\ref{fig:trans}.
Then, all nodes $\order_i$s in the ordering committee run a BO to agree on the sequence numbers in $\langle B_1, …, B_m\rangle$. 
Next, $\order_p$ sends each $B_i$ to the $i$th shard, where each executing node updates its local account states by executing the transactions in $B_i$, and returns the results in a {\em result block} to the ordering committee.
%all nodes process  in a single BFT round and update the transaction blockchain.

\remove{
\begin{figure}[htbp]
\small
\begin{mdframed}[leftline=false, rightline=false, linewidth=1pt, innerleftmargin=0cm, innerrightmargin=0cm]
\begin{algorithmic}[1]

%--------------------------------
\State \textbf{upon} reception of $\langle \trans_1, ..., \trans_k \rangle$ at $\order_p$ \textbf{do}
\State\label{101} \phantom{---} initiate $m$ empty blocks $\langle B_1, …, B_m\rangle$
\State\label{102}\phantom{----} \textbf{for} each $\trans_i$ in $\langle \trans_1, ..., \trans_k \rangle$
\State\label{103} \phantom{----}\phantom{----} \textbf{if} $\trans_i\in\Trans_1$
\State\label{104} \phantom{----}\phantom{----}\phantom{----} {\em singleShardTX}($\trans_i$)
\State\label{105} \phantom{----}\phantom{----} \textbf{else if} $\trans_i\in\Trans_2$
\State\label{106} \phantom{----}\phantom{----}\phantom{----} {\em crossShardIndependentTX}($\trans_i$)
\State\label{107} \phantom{----}\phantom{----} \textbf{else if} $\trans_i\in\Trans_3$
\State\label{108} \phantom{----}\phantom{----}\phantom{----} {\em crossShardDependencies}($\trans_i$)
\\
\Function{{\em singleShardTX}($\trans$)}{}
\State\label{109} \phantom{----} $j\leftarrow\trans_i$'s shard
\State\label{110} \phantom{----} $sn_j\leftarrow sn_j +1$
\State\label{111} \phantom{----} put $\langle TX, sn_j \rangle$ into $B_j$.
\EndFunction
\\
\Function{{\em crossShardIndependentTX}($\trans$)}{}
\State\phantom{----} Generate a set of preliminary transactions {\em prelTX}
\State\phantom{----} Generate a set of conclusory transactions {\em concTX}
\State\phantom{----} Cache {\em concTX}
\State\phantom{----} \textbf{for} each $\trans_i$ in {\em prelTX}
\State\label{120} \phantom{----}\phantom{----} {\em singleShardTX}($\trans_i$)
\EndFunction
\\
\Function{{\em crossShardDependencies}($\trans$)}{}
\State\phantom{----} Divide $\trans$ into a set of independent transactions {\em indTX}
\State\phantom{----} \textbf{for} each $\trans_i$ in {\em indTX}
\State\label{121} \phantom{----}\phantom{----} \textbf{if} $\trans_i\in\Trans_1$
\State\label{122} \phantom{----}\phantom{----}\phantom{----} {\em singleShardTX}($\trans_i$)
\State\label{123} \phantom{----}\phantom{----} \textbf{else if} $\trans_i\in\Trans_2$
\State\label{124} \phantom{----}\phantom{----}\phantom{----} {\em crossShardIndependentTX}($\trans_i$)
\EndFunction
%--------------------------------
\end{algorithmic}
\end{mdframed}
\caption{Pseudocode: transaction processing.}
\label{fig:trans}
\end{figure}
}


%in the following way: 
%for each transaction $\trans$, if it involves the $i$th shard  it increases $sn_i$ and puts $\langle \trans, sn_i\rangle$ into $B_i$. 

%In order to balance the load of the ordering committee, we allow 

%This strategy is sufficient to handle {\em independent transactions}, which represents atomic executions of single, one-shot code blocks across multiple shards~\cite{Cowling2012}.
%While independent transactions are useful, they do not capture all possible operations, 
%such as conditional update that depends on the data objects on another shard.
%Following Eris~\cite{Eris}, we use independent transactions as building blocks to execute {\em general transactions} that have cross-shard dependencies.  
%Namely, these general transactions are committed in two phases: in the first phase, the client sends a preliminary transaction, which executes the reads and acquires all read and write locks; in the second phase, the client sends a conclusory transaction, which either commits or aborts the transaction. When a shard member suspects that a client has failed because it has held locks for too long without sending the conclusory Commit or Abort, this member can unilaterally abort the transaction simply by sending the Abort command as an single transaction itself. 

\remove{
Our sharding protocol has two advantages over OmniLedger~\cite{Omniledger} and Chainspace~\cite{Chainspace}.
First, in our protocol, nodes do not need to run BFT within each shard. This improve the performance a lot.
Second, OmniLedger and  Chainspace suffer from the Denial-of-Service attacks. 
Our protocol has no such issue because both $\trans_A$ and $\trans_B$ will go to the ordering committee and be executed in the same order in both shards.
Regardless of the DoS attacks, our protocol also improves the success rates for such transactions.}




